code2seq: Generating Sequences from Structured Representations of Code

The ability to generate natural language sequences from source code snippets has a variety of applications such as code summarization, documentation, and retrieval. Sequence-to-sequence (seq2seq) models, adopted from neural machine translation (NMT), have achieved state-of-the-art performance on these tasks by treating source code as a sequence of tokens. We present ${\rm {\scriptsize CODE2SEQ}}$: an alternative approach that leverages the syntactic structure of programming languages to better encode source code. Our model represents a code snippet as the set of compositional paths in its abstract syntax tree (AST) and uses attention to select the relevant paths while decoding. We demonstrate the effectiveness of our approach for two tasks, two programming languages, and four datasets of up to $16$M examples. Our model significantly outperforms previous models that were specifically designed for programming languages, as well as state-of-the-art NMT models. An interactive online demo of our model is available at http://code2seq.org. Our code, data and trained models are available at http://github.com/tech-srl/code2seq.

==> genericmacros.tex <==
%!TEX root=draft.tex

% Generic macros (nothing specific to this paper)

\usepackage{ifthen}
%
\newcommand{\todoi}[1]{{\todo[inline]{#1}}}
\newcommand{\todolow}[1]{}
% \newcommand{\TODO}[1]{ {\color{blue} {\bf #1}} }
\newcommand{\TODO}[1]{ {\color{blue} \bf #1} }
\newcommand{\DONE}[1]{ {\color{gray} \textbf{DONE - } #1} }
\newcommand{\OMIT}[1]{ {\color{gray} \bf #1} }
\newcommand{\AWK}[1]{ {\color{red} \bf #1} }
\newcommand{\TODOFN}[1]{ \footnote{{\bf #1}} }
\newcommand{\COMMENT}[1]{}
\newcommand{\ignore}[1]{}
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}

%%% references definition
\newcommand{\lemref}[1]{Lemma~\ref{Lm:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{Fi:#1}}
\newcommand{\defref}[1]{Definition~\ref{De:#1}}
\newcommand{\theref}[1]{Theorem~\ref{Th:#1}}
\newcommand{\tabref}[1]{Table~\ref{Ta:#1}}
%\newcommand{\secref}[1]{Section~\ref{Se:#1}}
\newcommand{\secrefs}[2]{Sections~\ref{Se:#1}-\ref{Se:#2}}
\newcommand{\ssecref}[1]{Sec.~\ref{Se:#1}}
\newcommand{\appref}[1]{Appendix~\ref{Se:#1}}
\newcommand{\exref}[1]{Example~\ref{Ex:#1}}
\newcommand{\algref}[1]{Algorithm~\ref{Alg:#1}}
\newcommand{\lnref}[1]{Line~\ref{Ln:#1}}
\newcommand{\slnref}[1]{\ref{Ln:#1}}

\newcommand{\lemlabel}[1]{\label{Lm:#1}}
\newcommand{\figlabel}[1]{\label{Fi:#1}}
\newcommand{\deflabel}[1]{\label{De:#1}}
\newcommand{\thelabel}[1]{\label{Th:#1}}
\newcommand{\tablabel}[1]{\label{Ta:#1}}
\newcommand{\seclabel}[1]{\label{Se:#1}}
\newcommand{\sseclabel}[1]{\label{Se:#1}}
\newcommand{\applabel}[1]{\label{Se:#1}}
\newcommand{\exlabel}[1]{\label{Ex:#1}}
\newcommand{\alglabel}[1]{\label{Alg:#1}}
\newcommand{\lnlabel}[1]{\label{Ln:#1}}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[]

%% TO Allow writing the TR in the same source
\newboolean{TR}
\setboolean{TR}{false}
\ifthenelse{\boolean{TR}}{
\newcommand{\TrSelect}[2]{#1}
\newcommand{\TrOnly}[1]{#1}
\newcommand{\SubOnly}[1]{}
\newcommand{\TrOnlyInFootnote}[1]{#1}
\newcommand{\TrOnlyInTable}[1]{#1}}
{
\newcommand{\TrSelect}[2]{#2}
\newcommand{\TrOnly}[1]{}
\newcommand{\SubOnly}[1]{#1}
\newcommand{\TrOnlyInFootnote}[1]{}
\newcommand{\TrOnlyInTable}[1]{}}

%% General macros
\newcommand{\Set}[1]{\{ \; {#1} \; \}}
\newcommand{\vbar}{\; | \;}
\newcommand{\notIn}{\not\in}
\newcommand{\sizeof}[1]{|{#1}|}
%% \newcommand{\isDefined}{=_{def}}
\newcommand{\isDefined}{\triangleq}

\newcommand{\lt}{$<$}
\newcommand{\gt}{$>$}

%% tminus: "thin minus", with less space around it;
%% telem: "thin element"
\newcommand{\tminus}{\!\! - \!\!}
\newcommand{\telem}{\! \in \!}

%% stexttt: "small" texttt
\newcommand{\stexttt}[1]{{\small \texttt{#1}}}

\newcommand{\mathify}[1]{\mathord{\mbox{#1}}}
\newcommand{\italMathId}[1]{\mathify{\textit{\textrm{#1}}}}
\newcommand{\romanMathId}[1]{\mathify{\textup{\textrm{#1}}}}
\newcommand{\ttMathId}[1]{\mathify{\textup{\texttt{#1}}}}

\newcommand{\ttsub}[2]{${\ttMathId{#1}}_{#2}$}
\newcommand{\ttsup}[2]{${\ttMathId{#1}}^{#2}$}
\newcommand{\mttsub}[2]{{\ttMathId{#1}}_{#2}}
\newcommand{\twoarray[2]}{\begin{array}{l}  #1 \\ #2 \end{array}}


% \newcommand{\CBS}{\begin{leftbar}}
% \newcommand{\CBE}{\end{leftbar}}
\newcommand{\CBS}{}
\newcommand{\CBE}{}


%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}


==> packages.tex <==
%!TEX root=draft.tex
\usepackage[dvipsnames,usenames]{color}
\usepackage{fancyvrb}
\usepackage{setspace}
\usepackage{url}
\usepackage[dvipsnames]{xcolor}
\usepackage{paralist}
\usepackage[small,compact]{titlesec}
\usepackage{setspace}
\usepackage{times}
\usepackage{paralist}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage[geometry,clock]{ifsym}
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
\usepackage[dvipsnames,usenames]{color}
\usepackage{listings}
\usepackage{float}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{epsfig}
% A good source for fonts:
% http://tex.stackexchange.com/questions/213835/using-many-typewriter-fonts-in-a-single-document
\usepackage{txfonts}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{rotating}
\usepackage{mathpartir}
\usepackage{array}
\usepackage{todonotes}
\usepackage[percent]{overpic}
\usepackage{ragged2e}
\usepackage{fancybox}
%\usepackage{pstricks}
\usepackage{hyperref}
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{xspace} % makes sure we have spaces before next word, but not before punctuation.
\usepackage{lastpage}
%\usepackage{slashbox}
\usepackage{enumitem}
%\usepackage{enumerate}

\usepackage{mathtools} 

\usepackage{booktabs}


\usepackage{framed}




==> specificmacros.tex <==
%!TEX root=draft.tex

\newcommand{\EY}[2]{ {\color{red} #1 (\textbf{EY}: \emph{#2})} }
% \newcommand{\YD}[2]{ {\color{ForestGreen} #1 (\textbf{YD}: \emph{#2})} }
% \newcommand{\NP}[2]{ {\color{purple} #1 (\textbf{NP}: \emph{#2})} }

\newcommand{\tool}{\scode{GitZ}\xspace}

\newcommand{\demonsmarker}{\textbf{DEMONS START HERE, IF NOT EARLIER}}

\newcommand{\neighbrel}{\tilde{\delta}}
\newcommand{\neighb}[2]{\neighbrel(#1,#2)}

% programming languages
\newcommand{\Python}{\scode{Python}\xspace}
\newcommand{\CSharp}{\scode{C\#}\xspace}

% other
\newcommand{\Github}{\scode{Github}\xspace}

% text formatting
\newcommand{\sectionette}[1]{\vspace{1pt}\noindent \textit{#1}:}
\newcommand{\para}[1]{\vspace{3pt}\noindent\textbf{\textit{#1}}}
\newcommand{\scode}[1]{{\small \texttt{#1}}}
\newcommand{\tcode}[1]{{\scriptsize \texttt{#1}}}
\newcommand{\sname}[1]{{\small \textsc{#1}}}

% colors
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{blue(pigment)}{rgb}{0.2, 0.2, 0.6}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{carminered}{rgb}{1.0, 0.0, 0.22}
\definecolor{electricindigo}{rgb}{0.44, 0.0, 1.0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\hypersetup{colorlinks=true,linkcolor=black, citecolor=black, urlcolor=black}

\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.35} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc

%\definecolor{path-red}{HTML}{B85450}
%\definecolor{path-blue}{HTML}{6C8EBF}
\definecolor{path-orange}{HTML}{D79B00}
\definecolor{path-green}{HTML}{517040}

\usepackage{listings}
\lstset{language=Java,
    basicstyle=\ttfamily,
    keywordstyle=\color{javapurple}\bfseries,
    stringstyle=\color{javared},
    commentstyle=\color{javagreen},
    morecomment=[s][\color{javadocblue}]{/**}{*/},
    %numbers=left,
    numberstyle=\tiny\color{black},
    stepnumber=2,
    numbersep=10pt,
    tabsize=4,
    showspaces=false,
    showstringspaces=false,
    showlines=true
}

\newcommand{\rulesep}{\unskip\ \vrule\ }

% lstlistings styles
%\lstset{basicstyle=\ttfamily\scriptsize,
%        language=C,
%        emph={},
%        emphstyle={\underbar},
%        numbers=none,
%        numberfirstline=false,
%        numberstyle=\tiny\color{mygray},
%        escapeinside={(*@}{@*)}}

%\newcommand{\f1}{0.58}
\newcommand{\fscore}{$0.58$}


